Stateful Posted Pricing with Vanishing Regret via Dynamic Deterministic Markov Decision Processes

In this paper, a rather general online problem called dynamic resource allocation with capacity constraints (DRACC) is introduced and studied in the realm of posted price mechanisms. This problem subsumes several applications of stateful pricing, including but not limited to posted prices for online job scheduling and matching over a dynamic bipartite graph. As the existing online learning techniques do not yield vanishing-regret mechanisms for this problem, we develop a novel online learning framework defined over deterministic Markov decision processes with dynamic state transition and reward functions. We then prove that if the Markov decision process is guaranteed to admit an oracle that can simulate any given policy from any initial state with bounded loss -- a condition that is satisfied in the DRACC problem -- then the online learning problem can be solved with vanishing regret. Our proof technique is based on a reduction to online learning with switching cost, in which an online decision maker incurs an extra cost every time she switches from one arm to another. We formally demonstrate this connection and further show how DRACC can be used in our proposed applications of stateful pricing.

==> tex/PPP.tex <==

\subsubsection*{\emph{Application to the DRACC problem (continued):}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We can now use the C\&S algorithm (Algorithm~\ref{alg:chasing_and_switching}) for the special case of the DRACC problem. This final mechanism is called Learning Based Posted Pricing ({\MechanismName}). It first provides the input parameters of the C\&S algorithm, including the collection $\Gamma$ of one-shot pricing policies, the OLSC algorithm $\mathcal{A}$, the chasing ongoing oracle $\mathcal{O}^{\mathtt{Chasing}}$ and the initial state $s_{1}$. It then run the C\&S algorithm by posting its prices (actions) and updating the state ({\Surplus} vector). As for the chasing ongoing oracle, we rely on the particular choice of randomized $\mathcal{O}^{\mathtt{Chasing}}$ used in the proofs of \Cref{theorem_chasing_condition} for $k(t)$-demand users, and \Cref{theorem_chasing_condition-general} for the general case. As for the initial state,  we set $s_{1}$ to $\LVEC \MultiSym{i}\RVEC_{i \in A_1}$.


% As one last technical note, without loss of generality, we assume that $t_{a}(1) = 1$, because otherwise the {\Buyers} $i$ with $i < t_{a}(1)$ can never get any {\Item}. Therefore, the initial state $s_{0}$ can be specified by setting it to $\LVEC \MultiSym{i}\RVEC_{i \in A_1}$, and this can be done before the arrival of the first {\Buyer}.


% This section designs a learning-based posted price mechanism ({\MechanismName}) for the DRACC problem using the C\&S algorithm, and prove that this mechanism has vanishing regret. 

% The mechanism {\MechanismName} works as follows. It first provides the initial input parameters to the Algorithm C\&S, including the collection $\Gamma$ of policies, the OLSC algorithm $\mathcal{A}$, the chasing ongoing oracle $\mathcal{O}^{\mathtt{Chasing}}$ and the initial state $s_{0}$. In particular, the existence of the algorithm $\mathcal{A}$ is guaranteed in Lemma \ref{lemma_preliminary_on_ODSC}, and the desired chasing ongoing oracle $\mathcal{O}^{\mathtt{Chasing}}$ is constructed at the end of this section. Without loss of generality, we assume that $t_{a}(1) = 1$, because otherwise the {\Buyers} $i$ with $i < t_{a}(1)$ can never get any {\Item}. Therefore, the initial state $s_{0}$ can be specified by setting it to $\LVEC \MultiSym{i}\RVEC_{i \in A_1}$, and this can be done before the arrival of the first {\Buyer}.

% When the first {\Buyer} arrives, {\MechanismName} invokes C\&S to obtain the first action $x_{1} \in X_{s_{0}}$, and posts $x_{1}$ as the price vector for the {\Buyer} $t = 1$. Next, upon the arrival of each {\Buyer} $t \in [2, T]$, {\MechanismName} constructs the reward function $f_{t - 1}$ and the state transition function $g_{t - 1}$, which are described in detail later. After these two functions are fed to C\&S, C\&S chooses a new action $x_{t}$, and {\MechanismName} posts $x_{t}$ as the price vector for the {\Buyer} $t$. This process proceeds iteratively until all the $T$ {\Buyers} have been processed.





%Theorem \ref{theorem_chasing_condition} implies that the DRACC instance is $\sigma$-chaseable with $\sigma = \MaxMultiSym \cdot W$.
The following results can be directly inferred from Theorem~\ref{theorem_regret_of_hola} and Theorem~\ref{theorem_chasing_condition}, \Cref{theorem_chasing_condition-general}.

\begin{theorem}\label{theorem_regret_of_mechanism_for_BIT}
In the DRACC problem with $k$-demand user valuations, the regret of {\MechanismName} is bounded by
\begin{equation*}
O\Big( (\MaxMultiSym W)^{\frac{1}{4}} T^{\frac{3}{4}} \sqrt{\log |\PricePols|} \Big) \, .
\end{equation*}
\end{theorem}
\begin{theorem}\label{theorem_regret_of_mechanism_for_BIT_general}
In the DRACC problem with general user valuations, the regret of {\MechanismName} is bounded by
\begin{equation*}
O\Big( T^{\frac{1}{2}\left(1+\frac{CW}{CW+1}\right)} \sqrt{\log |\PricePols|} \Big) \, .
\end{equation*}
\end{theorem}

Notably, the guarantee that {\MechanismName} has vanishing regret requires the modeling assumption that $\MaxMultiSym \cdot W \cdot \log^{2} |\Gamma| = o(T)$. By contrast, no posted pricing mechanism can guarantee a sublinear regret when $\MaxMultiSym \cdot W = \Omega(T)$, as we prove in \Cref{section:assumption-necessity} in the appendix. See \Cref{theorem_impossibility_result_for_C_W} for more details.



==> tex/acm.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2018}
%\acmYear{2018}
%\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference{The Web Conference 2020}{April 20--24, 2020}{Taipei}
%\acmBooktitle{The Web Conference 2020,
%  April 20--24, 2020, Taipei}
%\acmPrice{15.00}
%\acmISBN{}

==> tex/bipartite-matching.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the online bipartite matching (BM) problem, there are two sets of nodes, which are denoted by $\LeftSet = \lbrace \LeftNode \rbrace_{\LeftNode \in \LeftInts}$ and $\RightSet = \lbrace \RightNode \rbrace_{\RightNode \in \RightInts}$, respectively. The nodes in each of these two sets arrive sequentially and dynamically. For each node $\LeftNode \in [|\LeftSet|]$, an adversary specifies a pair of parameters $t_{a}(\LeftNode) \in \RightInts$ and $t_{e}(\LeftNode) \in [t_{a}(\LeftNode), |\RightSet|]$. It means that the node $\LeftNode$ arrives just before the arrival of the node $t_{a}(\LeftNode) \in Y$, and expires immediately after the decision for the node $t_{e}(\LeftNode) \in Y$ has been made. 
For each $\RightNode \in \RightSet$, define $A_{\RightNode} = \lbrace \LeftNode \in \LeftSet: \RightNode \in [t_{a}(\LeftNode), t_{e}(\LeftNode)] \rbrace$. Let $w_{\RightNode} = |A_{\RightNode}|$, and $W = \max_{\RightNode}w_{\RightNode}$. The adversary also chooses a value $v_{\RightNode, \LeftNode} \in [0, 1)$ for each $\RightNode \in \RightSet$ and each $\LeftNode \in A_{\RightNode}$. The parameters $|\RightSet|$, $W$, as well as a finite set $P$ of prices in $(0, 1]$ with $1 \in P$ are revealed in advance.

A posted price mechanism should decide a price vector $\VEC{p}_{\RightNode} \in P^{w_{\RightNode}}$ when each node $\RightNode \in \RightSet$ arrives, without knowing any information of $v_{\RightNode}$. If there exists some $k \in [w_{\RightNode}]$ so that $v_{\RightNode}(A_{\RightNode}(k)) - \VEC{p}_{\RightNode}(k) \geq 0$, then the mechanism allocates the node $A_{\RightNode}(\FAVleftNode{\RightNode}{\VEC{p}_{\RightNode}})$ to $\RightNode$ where $\FAVleftNode{\RightNode}{\VEC{p}_{\RightNode}} = \operatorname{argmax}_{k \in w_{\RightNode}} v_{\RightNode}(A_{\RightNode}(k)) - \VEC{p}_{\RightNode}(k)$, and charges $\RightNode$ the payment $\VEC{p}_{\RightNode}(\FAVleftNode{\RightNode}{\VEC{p}_{\RightNode}})$. Otherwise, $\RightNode$ does not get any node $\LeftNode \in A_{\RightNode}$, and pays $0$. Immediately after the decision on the allocation of the node in $A_{\RightNode}$ to $\RightNode$ has been made, $\RightNode$ reports the values $\lbrace v_{\RightNode, \LeftNode} \rbrace_{\LeftNode \in A_{\RightNode}}$. The following additional assumptions are made for the nodes.
\begin{enumerate}
\item For each $\LeftNode < |\LeftSet|$,
\begin{equation*}
t_{a}(\LeftNode) \leq t_{a}(\LeftNode + 1) \, , \text{ and } \, t_{e}(\LeftNode) \leq t_{e}(\LeftNode + 1)
\end{equation*}
\item The parameter $W$ does not grow with the size of $\RightSet$.
\end{enumerate}

The BM problem requires that each node $\LeftNode \in \LeftSet$ can be allocated to at most one node $\RightNode \in \RightSet$, which implies that for every $\RightNode \in \RightSet$ and every $k \in w_{\RightNode}$, if $A_{\RightNode}(k)$ has been allocated to some $\RightNode' \in \RightSet$ with $\RightNode' < \RightNode$, then $\VEC{p}_{j}(k)$ should be set to $1$. The mechanism is allowed to utilize the random bits when specifying the price vectors, and its goal is to maximize the expected total payments obtained from the nodes in $\RightSet$. The set $\PricePols$ of pricing policies $\gamma$ and the regret are defined in the same way as the DRACC problem.

This problem can be transformed to a special case of the DRACC problem by taking the nodes in $\LeftSet$ (resp.~$\RightSet$) as the {\Items} (resp.~{\Buyers}). The {\Multiplicity} of every {\Item} is exactly one.  The valuation function of each {\Buyer} $\RightNode$ maps each single {\Item} $\LeftNode \in A_{\RightNode}$ to $v_{\RightNode, \LeftNode}$, while mapping any other subset of the {\Items} in $A_{\RightNode}$ to $0$. Using Theorem \ref{theorem_regret_of_mechanism_for_BIT}, we get the following result.

\begin{corollary}
For the BM problem, the regret of the PPP mechanism is bounded by $O\Big(\sqrt{|\RightSet| \cdot \log|\PricePols|}\Big)$.
\end{corollary}


==> tex/ccsxml.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003752.10010070.10010099.10010101</concept_id>
<concept_desc>Theory of computation~Algorithmic mechanism design</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010099.10010107</concept_id>
<concept_desc>Theory of computation~Computational pricing and auctions</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010071.10010079</concept_id>
<concept_desc>Theory of computation~Online learning theory</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070.10010071.10011194</concept_id>
<concept_desc>Theory of computation~Regret bounds</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation~Algorithmic mechanism design}
\ccsdesc[500]{Theory of computation~Computational pricing and auctions}
\ccsdesc[300]{Theory of computation~Online learning theory}
\ccsdesc[300]{Theory of computation~Regret bounds}


==> tex/lower-bounds-wrong.tex <==
\label{apx:lower}
In this part, we will prove lower bounds on the regret of online learning algorithms for $\sigma$-chasable Dd-MDP instances under the full-information setting and bandit setting, respectively.

\begin{theorem}\label{theorem_reduction_from_switching_cost}
The regret of any online learning algorithm for $\sigma$-chasable Dd-MDP under full-information (resp., bandit) feedback is lower bounded by  $\Omega(\sqrt{T \log |{\Gamma}|})$
(resp., $\Omega(|{\Gamma}|^{1/3}T^{2/3})$).
\end{theorem}

\begin{proof}
We only prove the full information lower bound, and the proof of the bandit version follows the same lines.
Suppose the statement of the theorem does not hold.
Then, there exists an online learning algorithm with regret of
$o(\sqrt{\sigma \cdot T \log |{\Gamma}|})$
for any $1$-chasable instance of the Dd-MDP problem.
We show how to use this algorithm to design an OLSC algorithm with a unit switching cost whose regret is
$o(\sqrt{\sigma \cdot T \log |\mathcal{X}|})$,
where $\mathcal{X}$ is the action set of the OLSC instance.
This is in contradiction to the known information theoretic 
$\Omega(\sqrt{\sigma \cdot T \log |\mathcal{X}|})$
lower bound on the regret of OLSC under the full-information setting \cite{Cesa2006PLG, Freund1995DTG, Littlestone1989WMA}.
(For the bandit version of this proof we use the lower bound of \cite{Dekel2014BSC}).
% To see this, fix an online learning algorithm for $1$-chasable Dd-MDP instances with $T$ {\Steps} and policy collection $\Gamma$ with regret $R(T, |\Gamma|)$.
% We show the OLSC problem with $T$ {\Steps} and action collection $\mathcal{X}$ admits an online learning algorithm with regret $O\Big( R(T, |\mathcal{X}|) \Big)$.

Here is how the reduction works:
Given an OLSC instance with a set $\mathcal{X}$ of actions and switching cost $\hat{\Delta}$, we construct a Dd-MDP instance with a set $S^{x}$ of $M$ states $\lbrace s_{i}^{x} \rbrace_{i \in [T]}$ for each action $x \in \mathcal{X}$, where $M > 0$ is a sufficiently large parameter whose value is determined later.
An arbitrary state $s \in S$ is selected to be the initial state $s_{1}$. Moreover, we set $\mathcal{X}_{s} = \mathcal{X}$ for every state $s$.
For every $x \in \mathcal{X}$, we introduce a policy $\gamma^{x}$ in the policy collection $\Gamma$ of the Dd-MDP, defined so that it maps all states to action $x \in \mathcal{X}$.
For each round $t$, when the adversary in OLSC specifies a reward function $F_{t}(\cdot)$, we construct the state transition function and reward function in the Dd-MDP by setting
\begin{align*}
    g_{t}(s_{i}^{x}, x') = \begin{cases}
    s_{\min\lbrace 1, i - 1\rbrace}^{x} & \text{if } x = x' \\
    s_{i - 1 + \Delta}^{x'} & \text{otherwise}
    \end{cases}
    \quad \text{and} \quad
    f_{t}(s_{i}^{x}, x') = \begin{cases}
    \frac{1}{2}F_{t}(x') & \text{if } x = x' \wedge i = 1 \\
    \frac{1}{2}F_{t}(x') + \frac{1}{2} & \text{otherwise}
    \end{cases}
\end{align*}
%\begin{equation*}
%    g_{t}(s, x) = s^{x}
%    \qquad \text{and} \qquad
 %   f_{t}(s, x) = \frac{1}{2}F_{t}(x) + \frac{1}{2} \cdot 1_{s = s^{x}} \, .
%\end{equation*}
Obviously, this is a $1$-chasable Dd-MDP instance.
Moreover,
\begin{equation*}
    \max_{\gamma^{x} \in \Gamma}\sum_{t \in [T]} f_{t}(\FPS{t}{\gamma^{x}}, \FPA{t}{\gamma^{x}}) - \sum_{t \in [T]} \mathbb{E}\Big[ f_{t}(s_{t}, x_{t}) \Big] \leq o(\sqrt{T\log|\Gamma|}) = o(\sqrt{T\log|\mathcal{X}|}) \, ,
\end{equation*}
where the inequality is due to the assumed regret bound.
The construction of the Dd-MDP instance ensures that for every $\gamma \in \Gamma$,
\begin{align*}
    \sum_{t \in [T]} f_{t}(\FPS{t}{\gamma^{x}}, \FPA{t}{\gamma^{x}}) \geq&  \, \frac{1}{2} \cdot \sum_{t \in [T]} F_{t}(x) + \frac{1}{2}(T - 1) \, ,\\
    \sum_{t \in [T]} f_{t}(s_{t}, x_{t}) \leq& \frac{1}{2} \sum_{t \in [T]} F_{t}(x_{t}) + \frac{1}{2}T - \frac{1}{2} \sum_{t \in [2, T]} 1_{x_{t} \neq x_{t-1}} \\
\end{align*}
Putting these pieces together, we get
\begin{equation*}
    \frac{1}{2}\bigg(\max_{x \in \mathcal{X}}\sum_{t \in [T]} F_{t}(x) - \sum_{t \in [T]} \mathbb{E}\Big[ F_{t}(x_{t}) \Big] + \sum_{t \in [2, T]}1_{x_{t} \neq x_{t - 1}}\bigg) - 1 \leq o\Big(\sqrt{T\log|\mathcal{X}|} \Big) \, ,
\end{equation*}
and therefore the regret of the OLSC instance is bounded by $o(\sqrt{T\log\lvert\mathcal{X}}\rvert)$, a contradiction.
\end{proof}



% \begin{corollary}
% The regret of any online learning algorithm for $1$-chasable Dd-MDP under full-information (resp. bandit information) is lower bounded by  $\Omega(\sqrt{T \log |{\Gamma}|})$ (resp.~$\Omega(|{\Gamma}$.
% (resp.~$\Omega(|{\Gamma}|^{1/3}T^{2/3})$).
% % Under the full-information setting (resp.~the bandit setting), the lower bound on the regret of online learning algorithms for $\sigma$-Chaseable Dd-MDP with some constant $\sigma > 0$ is $\Omega(\sqrt{T \log |{\Gamma}|})$ (resp.~$\Omega(|{\Gamma}|^{1/3}T^{2/3})$).
% \end{corollary}


==> tex/missing-proofs.tex <==
In this section, we provide the proofs missing from \cref{sec:main-technical}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of \cref{prop:no-noregret-general-DdMDP}]
Consider a simple scenario where there are only two states
$\lbrace s, s' \rbrace$
with $s$ being the initial state and two actions
$\lbrace x, x' \rbrace$
that are feasible for both states.
Without loss of generality, let $x$ be the action that the decision maker's algorithm chooses with probability at least
$1 / 2$
at time
$t = 1$.
Now, consider an adversary that works in the following manner:
It sets
$f_{t}(s, \cdot) = 1$
and
$f_{t}(s', \cdot) = 0$
for every
$t \in [T]$.
Regarding the state transition, the adversary sets
$g_{1}(s, x) = s'$
and
$g_{1}(s, x') = s$;
and for every
$t \in [2, T]$,
it sets
$g_{t}(s, \cdot) = s$
and
$g_{t}(s', \cdot) = s'$.
In such case, the expected cumulative reward of the decision maker is at most
$1 + T / 2$,
while the policy that always plays action $x_1$ obtains a cumulative reward of $T$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of \Cref{prop:deterministic-chasing-oracle}]
Consider an ongoing chasing oracle that is implemented in a deterministic manner for a DRACC instance with $\MaxMultiSym = 1$, $W = 2$. The adversary chooses initial step $\tinit$ and initial state $\sinit$ so that $\tinit = o(T)$, $|A_{\tinit}| = 2$, and $\VEC{\SurplusSym}_{\tinit} = \langle 0, 1 \rangle$. Note that throughout this proof, the {\Surplus} vectors and price vectors containing two elements are presented in an ordered way, which means that the first element corresponds to the {\Item} with the smaller index.

The target policy $\gamma$ is chosen to have $\FPremain{\tinit}{\gamma} = \langle 1, 1 \rangle$. Moreover, it maps every {\Surplus} vector to a price vector of $\langle \frac{2}{3}, \frac{1}{3} \rangle$. The adversary ensures the feasibility of such a policy by setting $t_{e}(i) = t$ for each {\Item} that is sold out at $t$ with the price vector generated by $\gamma$, and setting $t_{a}(i') = t + 1$ for a new {\Item}. With this setting, it holds for every $t \geq \tinit$ that $\FPremain{t}{\gamma} = \langle 1, 1 \rangle$.

The adversary configures the valuation functions $v_{t}$ for each $t \geq \tinit$ in an adaptive way, and ensures that for all such $t$
\begin{equation}
    \hat{\VEC{\SurplusSym}}_{t} = \langle 0, 1 \rangle \, . \label{formula_invariant_surplus_vector_for_deterministic_oracle}
\end{equation}
With the initial state $\sinit$ chosen by the adversary, Eq.~\eqref{formula_invariant_surplus_vector_for_deterministic_oracle} holds for $\tinit$. Suppose it holds for some $t \geq \tinit$. Then the price vector $\hat{\PriceVec}$ generated by the oracle must be in the form of $\langle 1, p \rangle$ for some $p \in (0, 1]$. Let $i$ and $i'$ be the two {\Items} in $A_{t}$ with $i < i'$. If $p \leq \frac{1}{3}$, the adversary sets $v_{t}(i) = \frac{2}{3}$ and $v_{t}(i') = \frac{1}{3}$. Then with the price vector generated by $\gamma$, payment $\frac{2}{3}$ is obtained from the {\Buyer} for {\Item} $i$, while the oracle obtains payment $\frac{1}{3}$ from the {\Buyer} for $i'$. The difference in rewards is
\begin{equation}
    f_{t}(\FPremain{t}{\gamma}, \FPprice{t}{\gamma}) - f_{t}(\hat{\VEC{\SurplusSym}}_{t}, \hat{\PriceVec}_{t}) = \frac{1}{3} \, . \label{formula_difference_in_payments_for_deterministic_oracle}
\end{equation}
Moreover, since $i$ is sold out with $\FPprice{t}{\gamma}$, the adversary sets $t_{e}(i) = t$ and $t_{a}(i'') = t + 1$ for a new {\Item} $i'' > i'$. In such case, it is guaranteed that Eq.~\eqref{formula_invariant_surplus_vector_for_deterministic_oracle} holds for $t + 1$.

For the case where $p > \frac{1}{3}$, it can be verified that Eq.~\eqref{formula_difference_in_payments_for_deterministic_oracle} still holds for $t$ and Eq.~\eqref{formula_invariant_surplus_vector_for_deterministic_oracle}  holds for $t + 1$ when the adversary sets $v_{t}(i) = v_{t}(i') = \frac{1}{3}$. Since Eq.~\eqref{formula_difference_in_payments_for_deterministic_oracle} is established for every $t \geq \tinit$, $CR = \frac{1}{3}(\tfinal - \tinit)$. With $\tinit = o(T)$, taking $\tfinal = T$ gives the desired bound.
\end{proof}


==> tex/neur-impact.tex <==
\label{section:neur_impact}

%\textcolor{red}{\textbf{TODO}}

%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
%biases in the data. If authors believe this is not applicable to them, authors can simply state this.

%Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

The authors believe that the broader impact question is not applicable to the current paper.

==> tex/prelim-online-learning.tex <==
\label{section:online-learning-dMDP}







==> tex/scheduling.tex <==
\label{subsection_online_job_scheduling}

In the JS problem, there are $J$ jobs arriving in an online fashion over $N$ {\Slots}. Each {\Slot} $i \in [N]$ is associated with a {\Bandwidth} $b(i)$, which means that this {\Slot} can be allocated to at most $b(i)$ jobs. For each job $j \in J$, an adversary specifies an arrival time $a_{j} \in [N]$, a deadline $d_{j} \in [a_{j}, N]$, a length $\lth_{j} \in [d_{j} - a_{j} + 1]$, and a value $v_{j} \in [0, 1)$ in advance. 
A mechanism for the JS problem presents a payment $p_{j}$ to each job $j \in [J]$ upon the arrival of $j$. The job $j$ is accepted if $v_{j} \geq p_{j}$. In such case, the mechanism allocates $\lth_{j}$ consecutive {\Slots} in the interval $[a_{j}, d_{j}]$ to $j$, and charges $j$ the payment $p_{j}$. Otherwise the job $j$ is rejected. The goal of the mechanism is to maximize the revenue, which refers to the total payments of the accepted jobs. 
Let $B = \max_{i \in [N]}b(i)$, and $W = \max_{j \in [J]} d_{j} - a_{j} + 1$. The parameters $J$, $B$, $W$, and a finite set $P$ of prices in $(0, 1]$ with $1 \in P$ are given at the beginning at the input, while $\lbrace b(i) \rbrace_{i \in [N]}$ and the parameters of the jobs are revealed dynamically.

In particular, at the beginning of each {\Slot} $i \in [N]$, the {\Bandwidth} $b(i + W - 1)$ is revealed when $i \in (1, N + 1 - W]$, while the {\Bandwidths} $\lbrace b(i') \rbrace_{i' \in [W]}$ of all the $W$-first {\Slots} are revealed when $i = 1$. Immediately after that, the set $J_{i} = \lbrace j: a_{j} = i \rbrace$ of jobs arrive in the system. A posted price mechanism for the JS problem is required to present a price vector $\VEC{p}_{j} \in P^{W}$ of length $W$ for each arrival job $j \in J_{i}$ without knowing anything about $\lbrace d_{j}, \lth_{j}, v_{j} \rbrace$. The utility of a job $j$ by choosing an interval $[i, i + \lth_{j} - 1] \subseteq [a_{j}, d_{j}]$ of $\lth_{j}$ consecutive {\Slots} with respect to any given price vector $\VEC{p}$ is denoted by
\begin{equation*}
\Utility{j}{i}{\VEC{p}} = v_{j} - \sum_{i' = i}^{i + \lth_{j} - 1}\VEC{p}(i' - a_{j} + 1) \, .
\end{equation*}
Let $\FAVstartSlot{j}{\VEC{p}_{j}} = \operatorname{argmax}_{i \in [a_{j}, d_{j} - \lth_{j} + 1]}\Utility{j}{i}{\VEC{p}}$, and ties are broken by choosing the earliest {\Slot}. If $\Utility{j}{\FAVstartSlot{j}{\VEC{p}_{j}}}{\VEC{p}_{j}} \geq 0$, then the mechanism allocates $j$ to $[\FAVstartSlot{j}{\VEC{p}_{j}}, \FAVstartSlot{j}{\VEC{p}_{j}} + \lth_{j} - 1]$, and charges $j$ by $\ChoicePayment{j}{\VEC{p}_{j}} = \sum_{i' = \FAVstartSlot{j}{\VEC{p}_{j}}}^{\FAVstartSlot{j}{\VEC{p}_{j}} + \lth_{j} - 1}\VEC{p}_{j}(i)$. Otherwise, the job $j$ takes no {\Slot}, and its payment $\ChoicePayment{j}{\VEC{p}_{j}} = 0$. Immediately after that, the job $j$ reports its parameters $\lbrace d_{j}, \lth_{j}, v_{j} \rbrace$ to the mechanism. The mechanism is allowed to use random bits when deciding the price vectors $\lbrace p_{j} \rbrace_{j \in [J]}$, and its goal is to maximize the expected revenue $\sum_{j \in [J]}\mathbb{E}\big[ \ChoicePayment{j}{\VEC{p}_{j}} \big]$.

For every job $j \in [J]$, let $w_{j} = \min\lbrace W, N + 1 - a_{j} \rbrace$. Recall that the {\Bandwidths} of the {\Slots} in $[a_{j}, a_{j} + w_{j} - 1]$ have been known upon the arrival of $j$. Let $\VEC{l}_{j}$ and $\VEC{\SurplusSym}_{j}$ be two $w_{j}$-dimensional vectors so that for each $k \in [w_{j}]$, $\VEC{l}_{j}(k)$ represents the number of jobs in $[j - 1]$ that the {\Slot} $a_{j} + k - 1$ is allocated to, and $\VEC{\SurplusSym}_{j}(k) = b(a_{j} + k - 1) - \VEC{l}_{j}(k)$. A price vector $\VEC{p}_{j}$ is said to be feasible for $\VEC{\SurplusSym}_{j}$ if for every $k \in [w_{j}]$ with $\VEC{\SurplusSym}_{j}(k) = 0$, $\VEC{p}_{j}(k)$ is set to $1$. It is required that for every $j \in [J]$, the price vector $\VEC{p}_{j}$ posted by the mechanism should be feasible for $\VEC{\SurplusSym}_{j}$ so that the constraint on the {\Bandwidth} is not violated. Also, every pricing policy $\gamma \in \PricePols$ should map every possible {\Surplus} vector $\VEC{\SurplusSym}$ to a price vector $\VEC{p}$ of the same length so that $\VEC{p}$ is feasible for $\VEC{\SurplusSym}$. Let $\FPprice{j}{\gamma}$ be the price vector given by $\gamma$ for job $j$ after inductively applying $\gamma$ to the jobs in $[j - 1]$, the regret of a mechanism for JS is defined to be
\begin{equation*}
\max_{\gamma}\sum_{j \in [J]} \ChoicePayment{j}{\gamma} - \sum_{j \in [J]}\mathbb{E}\big[\ChoicePayment{j}{\VEC{p}_{j}} \big] \, ,
\end{equation*} 
where $\ChoicePayment{j}{\gamma}$ is the shorthand of $\ChoicePayment{j}{\FPprice{j}{\gamma}}$. For this JS problem, we make the assumption that $B$ and $W$ do not increase with the number $J$ of jobs.

\PARA{Transformation to the DRACC problem}. Now we show that an instance of the JS problem can be transformed into a DRACC instance in an online manner. At the beginning, we set the number of {\Buyers} to $J$, and the number of {\Items} to $N$ to initialize the DRACC instance. It means that every job is viewed as a {\Buyer}, while each {\Slot} $i$ is taken as a {\Item} with {\Multiplicity} $\MultiSym{i} = b(i)$. The major problem in this part is to decide the arrival time $t_{a}(i)$ and the expiration time $t_{e}(i)$ of every {\Slot} $i \in [N]$. 

Fix a {\Slot} $i$ with $J_{i} \neq \emptyset$. For every {\Slot} $k \geq i$ whose {\Bandwidth} $b(k)$ has been revealed, if $\max\lbrace 1, k - W + 1 \rbrace > i - 1$, or for every $i' \in [\max\lbrace 1, k - W + 1 \rbrace, i - 1]$ we have $J_{i'} = \emptyset$, then we set $t_{a}(k) = \min\lbrace j \in J_{i}\rbrace$. This setting ensures that for every {\Slot} $i$, if there exists some job $j$ so that $i \in [a_{j}, a_{j} + w_{j} - 1]$, the arrival of $i$ is reported exactly once. It further implies that for every {\Slot} $i$ that has reported its arrival, there exists at least one {\Slot} $i' \in [\max\lbrace 1, i - W + 1 \rbrace, i]$ which satisfies $J_{i'} \neq \emptyset$. Then the expiration time $t_{e}(i)$ of such a {\Slot} $i$ is set to $\max\Big\lbrace j \in J_{i'}: i' \leq i \bigwedge J_{i'} \neq \emptyset \Big\rbrace$. In this way, a feasible instance of the DRACC problem can be obtained. The following result can be directly inferred from Theorem \ref{theorem_regret_of_mechanism_for_BIT}.

\begin{corollary}\label{corollary_regret_of_JS}
When applying the PPP mechanism to the JS problem, the regret is bounded by $O\big( \sqrt{J \cdot \log |\PricePols|} \big)$.
\end{corollary}


